Unifying Theories of Reactive Design Contracts

Design-by-contract is an important technique for model-based design in which a composite system is specified by a collection of contracts that specify the behavioural assumptions and guarantees of each component. In this paper, we describe a unifying theory for reactive design contracts that provides the basis for modelling and verification of reactive systems. We provide a language for expression and composition of contracts that is supported by a rich calculational theory. In contrast with other semantic models in the literature, our theory of contracts allow us to specify both the evolution of state variables and the permissible interactions with the environment. Moreover, our model of interaction is abstract, and supports, for instance, discrete time, continuous time, and hybrid computational models. Being based in Unifying Theories of Programming (UTP), our theory can be composed with further computational theories to support semantics for multi-paradigm languages. Practical reasoning support is provided via our proof framework, Isabelle/UTP, including a proof tactic that reduces a conjecture about a reactive program to three predicates, symbolically characterising its assumptions and guarantees about intermediate and final observations. This allows us to verify programs with a large or infinite state space. Our work advances the state-of-the-art in semantics for reactive languages, description of their contractual specifications, and compositional verification.

==> sec/background.tex <==
\subsection{Unifying Theories of Programming}

Programming and modelling languages often encompass a number of paradigms that are used to variously abstract the
world. Whilst general purpose languages exist which allow programming in any paradigm, such as object oriented,
concurrent, real-time, hybrid, and functional, domain specific languages are more conservative, encapsulating only one
or two. Unifying Theories of Programming (UTP) is a framework for formalisation and combination of theories that
underlie the foundational semantics of programming languages. A UTP theory, in this context, encapsulates a set of laws
that characterise a particular paradigmatic aspect of a language. For instance, one can identify a UTP theory for
real-time programs where a clock can be observed that provides information about the duration of a
computation.

In UTP, programs and models are encoded using a language of alphabetised predicates, following the
``programs-as-predicates'' philosophy. Reasoning about the behaviour of a program thus reduces to deduction in formal
logic, which provides us with a way of proving the laws of programming. UTP is therefore fundamentally denotational in
nature, since every programming language construct can be formally defined in terms of logical constructs, such as
conjunction, negation, and quantification. For example, it is well known that the imperative programming operators of
assignment, sequential composition, and the if-then-else conditional (written here in infix notation) can be logically
denoted as below:

\begin{definition}[Imperative programming constructs]
  \label{def:imper}
  \begin{align*}
    x := v       & ~~\triangleq~~ x' = v \land y_1' = y_1 \land \cdots \land y_n' = y_n \\[.5ex]
    P \relsemi Q & ~~\triangleq~~ \exists x_0 @ P[x_0/x'] \land Q[x_0/x] \\[.5ex]
    \conditional{P}{b}{Q} & ~~ \triangleq~~ (b \wedge P) \vee (\neg b \wedge Q)
  \end{align*}
\end{definition}

Such definitions give us a natural model for the algebraic laws of programming~\cite{Hoare87}, which can then be
employed in building programming verification tools~\cite{Armstrong2015}. Indeed programs-as-predicates is a very
natural fit to theorem proving since proof about a program reduces to a problem in Higher-Order Logic, which can often
be discharged using automated theorem proving, a fact we harness in our Isabelle-based UTP theorem prover,
Isabelle/UTP~\cite{Foster16b}. All the algebraic laws presented in this paper have been verified in Isabelle/UTP.

Going beyond simple imperative programs require that we consider UTP theories, that enrich the language of relations.
Concretely, a UTP theory consists of (1) a set of observational variables $A$ (the alphabet); (2) a set of healthiness
conditions; and (3) a signature. In order to exemplify, we will create a simple UTP theory of time $\theory{T}$. The
alphabet denotes the aspects of the world we wish to observe in the particular abstract setting. For example, theory
$\theory{T}$ could have variables $time, time' : \mathbb{R}$ that give the time before and after a
computation. Conversely, there are often situations when we may wish to abstract time, and may want to elide such a
variable. This is essence of the UTP's empirical approach: isolating aspects of the universe that we are interested in
to solve a particular problem.

The healthiness conditions denote invariants on the observational variables that define the correct behaviour of the
universe. Continuing our example, a possible healthiness condition is $time \le time'$, which means that the clock
cannot run backwards, which reflects our intuition of how time behaves. The signature of the theory consists of
constructs for building models that are healthy theory elements. For example, we might have a construct
$$\textbf{Wait}(n) \defs time' = time + n \land \II_{A \setminus \{time\}}$$ which introduces a delay of $n$ seconds.

Healthiness conditions, $\healthy{H}$, in UTP are expressed on functions on predicates, which should usually be (1)
idempotent and (2) monotone. Such a healthiness function when applied to a predicate yields a ``healthy'' predicate,
that is a valid element of the UTP theory. A predicate which satisfies $P = \healthy{H}(P)$ is called
$\healthy{H}$-healthy: it is a fixed point of $\healthy{H}$. Idempotence, defined as $\healthy{H} \circ \healthy{H} =
\healthy{H}$, means that application of a healthiness function need only be done once, and the resulting predicate
cannot be made more healthy. Monotonicity, defined as $P \sqsubseteq Q \implies \healthy{H}(P) \sqsubseteq
\healthy{H}(Q)$, means that the healthiness function preserves the refinement order on the original predicate. In our
theory of time, we can define our healthiness condition as $HT(P) = time \le time' \land P$, the application of which
restricts a predicate to healthy behaviours. $HT$ is both idempotent, since $time \le time' \land time \le time' \land P
= time \le time' \land P$, and also monotone since $\land$ is monotone.


\subsection{Design-by-Contract}

Design-by-Contract~\cite{Meyer92,Jones2003,Bauer2012} (DbC) is a compositional program construction and verification
technique. In DbC, one demonstrates composite system level properties by decomposing them into a number of contracts for
each component subsystem. Each contract specifies the guarantees that the subsystem will make about its behaviour, under
certain specified assumptions on the subsystem's environment. Meyer~\cite{Meyer92} coined the term when arguing the need
for precisely specified behavioural assertions about a program's behaviour to ensure reliability of component based
software systems. These assertions come in three forms: preconditions, postconditions, and invariants.

Meyer's work has its foundation in the work of Floyd~\cite{Floyd67} and Hoare~\cite{Hoare69} on proving correctness of
programs in terms of the commonly known Hoare triple $\lamporttriple{p}{Q}{r}$. This asserts that if program $Q$ is
started in a state satisfying predicate $p$ then, provided the program terminates, the final state will satisfy
predicate $r$. Effectively the Hoare triple is setting up a primitive contract for $Q$ that mandates a particular
relationship between inputs and outputs.

DbC is perhaps even more clearly seen in the work on refinement calculus~\cite{Mor1990}. Here, a programming language is
extended with a specification statement $w:[pre, post]$, where $pre$ is the precondition, $post$ the postcondition, and
$w$ the ``frame'' -- that is the set of variables that are allowed to change. A specification statement is to be
converted into a block of executable code through a series of correctness preserving refinements that variously divide
the specification into constituent parts, and eventually to atomic commands. Both Hoare logic and the refinement
calculus can be unified either algebraically~\cite{Gomes2016} or else denotationally using the UTP theory of
designs~\cite{Hoare&98}, which we discuss in Section~\ref{sec:designs}.

Moving beyond imperative programs to concurrent and reactive behaviours, where assumptions and guarantees range over the
entire history of interaction and not simply initial and final states, requires a richer form of
contract~\cite{Benveniste2007,Bauer2012,Champion2016}. Benveniste et al.~\cite{Benveniste2007} describe contracts
denotationally as pairs of predicates $C \defs (A, G)$ where $A$ is the assumption, and $G$ is the guarantee. $A$ and
$G$ both characterise the set of program variable traces that prescribe valid behaviours of the context and given
component, respectively. They define a notion of refinement, $C_1 \preceq C_2$ called dominance --- to distinguish it
from refinement to implementation -- which requires that the assumption be weakened and guarantee be strengthened. They
also define an algebra for contracts including parallel composition $C_1 \parallel C_2$, disjunction $C_1 \sqcap C_2$,
and conjunction $C_1 \sqcup C_2$. Works building on this framework~\cite{Cimatti2012,Cimatti2015} allow step-wise
refinement of contracts, and verification based on temporal logic properties. It is this notion of reactive contract
that our work speaks into.

\subsection{Designs}
\label{sec:designs}

The UTP theory of designs~\cite{Hoare&98,Cavalcanti&06} allows the specification of programs in a contractual manner in
terms of assumptions and guarantees, which we also call commitments. The theory has two observational variables,
$ok, ok' : \Bool$, flags that denote whether a program was started and whether it terminated, respectively. The
signature of the theory of designs consists of the operator $\design{P}{Q}$, that means that if a program is started and
the state satisfies assumption $P$, then it will terminate and satisfy commitment $Q$. This is denoted as follows:
\begin{definition}{Designs}
  \begin{align*}
    \design{P}{Q}   ~~\defs~~& (ok \land P) \implies (ok' \land Q)
  \end{align*}
\end{definition}
\noindent Here, $P$ and $Q$ are both relations on variables excluding $ok$ and $ok'$. Effectively this encoding allows a
pair of predicates to be encoded as a single predicate, such that designs effectively implement Benveniste's contract
framework~\cite{Benveniste2007}. We can thus define functions $\preD{D}$ and $\postD{D}$ that extracts the assumptions
and commitments, respectively, from a design, such that

$$\preD{P \shows Q} = P \quad\textrm{and}\quad \postD{P \shows Q} = (P \implies Q)$$

Designs are closed under sequential composition, disjunction, and conjunction, the latter of which give rise to near
identical operators present in~\cite{Benveniste2007}. Indeed, it is possible to prove the definitions of their operators
as theorems. Moreover, refinement of two designs $\design{P_1}{P_2} \refinedby \design{Q_1}{Q_2}$ requires that we can
demonstrate $P_1 \implies Q_1$ and $Q_2 \land P_1 \implies P_2$, that is we weaken the assumption and strengthen the
commitment. The theory of designs is therefore a very natural contract theory.

The healthiness conditions of designs characterise the associated UTP theory, and are given
below~\cite{Hoare&98,Cavalcanti&06}.
\begin{definition}{Design Healthiness Conditions}
  \begin{align*}
    \healthy{H1}(P) ~~\defs~~& (ok \implies P) \\
    \healthy{H2}(P) ~~\defs~~& P \relsemi \ckey{J} \\
    \ckey{J}        ~~\defs~~& ((ok \implies ok') \land \II_{A \setminus \{ok\}}) \\
    \healthy{H3}(P) ~~\defs~~& P \relsemi \IID \\
    \IID            ~~\defs~~& \design{\true}{\II} \\
    \healthy{H} &= \healthy{H1} \circ \healthy{H2} \\
    \healthy{N} &= \healthy{H1} \circ \healthy{H3}
  \end{align*}
\end{definition}
Designs are fixed-points of the healthiness condition $\healthy{H}$ which is composed of $\healthy{H1}$ and
$\healthy{H2}$. $\healthy{H1}$ states that until a design has been given permission to execute via $ok$, no observations
are possible. $\healthy{H2}$ states that no design can require non-termination. A more intuitive form that characterises
fixed-points is $P[false/ok'] \implies P[true/ok']$: every non-terminating behaviour for which $ok' = false$ has an
equivalent terminating behaviour for which $ok' = true$. $\healthy{H3}$ designs additionally require that $P$ is a
condition: it does not refer to dashed variables. The latter subclass is useful for ``normal'' specifications where the
assumption does not refer to the final state. $\ckey{H3}$ designs, with a few notable exceptions, are the most common
form of design, and are thus sometimes known as \emph{normal designs}~\cite{Guttman2010}, as indicated by healthiness
condition $\healthy{N}$.

The following theorems then demonstrate the relationship between syntactic designs and the healthiness conditions.

\begin{theorem}{Design correspondences}
  \begin{align*}
    \healthy{H}(P) &= \design{\preD{P}}{\postD{P}} \\
    \healthy{N}(P) &= \design{(\preD{P} \relsemi \true)}{\preD{P}}
  \end{align*}
\end{theorem}

Any $\healthy{H}$ predicate can thus be written using the design turnstile, if the precondition and postcondition are
extracted. Moreover, an $\healthy{N}$ predicate is a design whose precondition has $\true$ as a right unit and thus does
it does not refer to dashed variables. Designs allow us to unify various assertional reasoning techniques, notably Hoare
logic and refinement calculus, as shown below:
\begin{align*}
  \lamporttriple{p}{Q}{r} &~~\defs~~ (\design{p}{r} \refinedby Q) \\
  w:[pre, post] &~~\defs~~ (\design{pre}{post \land \II_{A \setminus w}})
\end{align*}
\noindent Designs are therefore an extremely versatile specification mechanism providing support for a number
verification techniques. 

\subsection{Generalised Reactive Processes}
\label{sec:bg-grp}

The theory of reactive processes~\cite{Hoare&98,Cavalcanti&06} unifies the semantics of different reactive
languages. Reactive languages differ from imperative programs in that they have intermediate observable states as well
as final states, where the process awaits interactions from its environment. The UTP theory of reactive processes has,
in addition to $ok$ and $ok'$, three pairs of observational variables $wait, wait' : \Bool$ that determine whether a
process (or its predecessor) is waiting for interaction with its environment or else has terminated,
$tr, tr' : \seq\,\textit{Event}$ that describes the trace before and after the process' execution, and
$ref, ref' : \power \textit{Event}$ that describe the events being refused during an intermediate state, as required by
the failures model of CSP~\cite{Hoare85}.

In our previous work~\cite{Foster17a} we have shown how the UTP theory of reactive processes can be generalised by
characterising the trace model with an abstract algebra, called a \emph{trace algebra}. From these algebraic foundations
we have reconstructed the complete theory of reactive processes, including its healthiness conditions and associated
laws, in particular those for sequential and parallel composition.

\begin{definition}[Trace algebra] \label{def:tralg} A trace algebra $(\tset, \tcat, \tempty)$ is a cancellative monoid
  satisfying the following the axioms:
\begin{align*}
  x \tcat (y \tcat z) &~=~ (x \tcat y) \tcat z \tag{TA1} \\
  \tempty \tcat x = x \tcat \tempty &= x \tag{TA2} \label{law:tunit} \\
  x \tcat y = x \tcat z ~~\implies~~  y &= z \tag{TA3} \label{law:tcancl1} \\
  x \tcat z = y \tcat z ~~\implies~~  x &= y \tag{TA4} \label{law:tcancl2} \\
  x \tcat y = \tempty  ~~\implies~~  x &= \tempty \tag{TA5} \label{law:tnai}
\end{align*}
\end{definition}

\noindent Operator $s \tcat t$ denotes trace concatenation, and $\tempty$ the empty trace. From these definitions and
axioms the usual operations of trace prefix ($s \le t$) and subtraction ($s - t$) can be derived and usual algebraic
laws proved as theorems~\cite{Foster17a}. Naturally, sequences are a model of the trace algebra, as are, for example,
piecewise continuous trajectories that are the basis of the denotational semantics of hybrid systems. From the trace
algebra we recreate the three reactive healthiness conditions.
\begin{definition} Reactive healthiness conditions
  \begin{align*}
    \healthy{R1}(P) & \defs P \land tr \le tr' \\
    \healthy{R2}_c(P) & \defs \conditional{P[\tempty, tr' \tminus tr/tr, tr']}{tr \le tr'}{P} \\
    \healthy{R3}(P) & \defs \conditional{\II}{wait}{P} \\
    \healthy{R} & \defs \healthy{R3} \circ \healthy{R2}_c \circ \healthy{R1}
  \end{align*}
\end{definition}
$\healthy{R1}$ states that $tr$ is monotonically increasing; processes are not permitted to undo past
events. $\healthy{R2}_c$ states that a process must be history independent: the only part of the trace it may constrain
is $tr' \tminus tr$, that it, the portion since the previous observation $tr$. Specifically, if the history is deleted,
by substituting $\tempty$ for $tr$ and $tr' - tr$ for $tr'$, then the behaviour of the process is unchanged. Our
formulation of $\healthy{R2}_c$ deletes the history only when $tr \le tr'$, which ensures that $\healthy{R2}_c$ does not
depend on $\healthy{R1}$, and thus commutes with it. Finally, $\healthy{R3}$ states that if a prior process is
intermediate ($wait'$) then the current process must identify all variables. We then compose the three to yield
$\healthy{R}$, the overall healthiness condition of reactive processes.

\subsection{Reactive Designs}

The UTP theory of reactive designs is an important foundation for reactive contracts that we will extend and elaborate
in this work. A reactive design is essentially a predicate that has all the healthiness conditions for both the design
theory ($\healthy{H}$) and the reactive process theory ($\healthy{R}$). Alternatively, a reactive design can be
characterised as a design which is make reactive: $\healthy{R}(\design{P}{Q})$, where $P$ is an assumption and $Q$ a
commitment, both of which can potentially refer to both state variables and the trace.

Designs and reactive processes are disjoint theories because $\healthy{H1}$ does not commute with either $\healthy{R1}$
or $\healthy{R3}$. Consequently, the order in which the healthiness conditions are applied is important: $\healthy{R3}$
must be applied first, followed by $\healthy{H1}$, and finally $\healthy{R1}$. The order of application of
$\healthy{H2}$ and $\healthy{R2}$ not important. In order to overcome the need for a specific order, the theory of
reactive designs introduces three derived healthiness conditions.

\begin{definition}
  \begin{align*}
    \healthy{CSP1}(P) ~\defs~& P \lor \neg ok \land (tr \le tr') \\
    \healthy{CSP2}(P) ~\defs~& \healthy{H2}(P) \\
    \healthy{R3}_c(P) ~\defs~& \conditional{\healthy{CSP1}(\II)}{wait}{P}
  \end{align*}
\end{definition}

\noindent $\healthy{CSP1}$ is equivalent to $\healthy{H1} \circ \healthy{R1}$, and unlike $\healthy{H1}$ does commute
with $\healthy{R1}$. Intuitively, $\healthy{CSP1}$ states that if $ok$ is not true, and thus we do not have permission
to execute, then the only predictable behaviour is that the trace must monotonically increase. Thus if a predecessor
commits erroneous behaviour ($\neg ok'$) through, for instance, having is assumption violated, then future behaviour is
unpredictable. $\healthy{CSP2}$ is simply $\healthy{H2}$, though with the alphabet extended with the reactive
observational variables. $\healthy{R3}_c$ is $\healthy{R3}$, but where the skip operator is made $\healthy{CSP1}$
healthy. In the UTP book~\cite{Hoare&98}, $\healthy{R3}_c$ is simply called $\healthy{R3}$, but their operator overloads
$\II$ to be either the operator we give here, or else the version of $\healthy{R3}$ we described in
section~\ref{sec:bg-grp}, which are both needed depending on whether one would like to handle divergence or not.

To exemplify reactive designs, consider the semantics of the simple assignment $x := f(e)$. It could be given as the
design $e \in \dom(f) \shows x' = f(e) \land y' = y$, for a program that has two programming variables $x$ and $y$. This
is not a reactive process, since it is not reactive-healthy: it executes even in its predecessor's wait-state. We can
make reactive-healthy by applying the appropriate reactive heathiness conditions. Here, we need both $\healthy{R1}$ and
$\healthy{R3}_c$. The result, $\healthy{R1} \circ \healthy{R3}_c(e \in \dom f \shows x' = f(e) \land y' = y)$, is a
reactive design. In general, we also apply $\healthy{R2}_c$ to ensure that the inner design does not attempt to observe
the trace history, though in this case $e \in \dom f \shows x' = f(e) \land y' = y$ is already $\healthy{R2}_c$
healthy. It would also be useful to go one step further and add the equality $tr' = tr$ to the postcondition before we
apply $\healthy{R}$ so that the trace is unchanged by the assignment, without this its behaviour is unpredictable beyond
$tr \le tr'$. The pay-off here is to add the theory of contracts provided by designs to the theory of reactive
processes, and in doing so extend its applicability to all the constructs found in common process algebras, including
parallel composition of processes, non-terminating recursive processes, channel communications, and abstraction
constructs including concealment of communications.

The idea of a reactive design as a semantic concept in its own right is a direct consequence of a result due to Hoare \&
He~\cite[Theorem 8.2.2]{Hoare&98}. This theorem states that CSP processes form a lattice closed under sequential
composition and containing the assignment $\healthy{R}(x:=e)$, for stored program variables $x$ and expressions $e$ over
these variables and suitable constants. The proof of the first claim is outlined by noting that $P$ is a CSP process
(that is, it satisfies the CSP healthiness conditions) iff
$$
  P = \healthy{R1}(\lnot P[false/wait,false/ok'] \shows P[false/wait,true/ok'])
$$
That is, every CSP-healthy process can be expressed as a design made reactive-healthy.

Cavalcanti \& Woodcock~\cite{Cavalcanti&06} discuss how this theorem accounts for a style of specification for CSP
processes, where the precondition of the design characterises the process's divergences and its postcondition describes
its failures (in the CSP sense). This paper also casts the semantics of some individual operators as reactive designs,
notably external choice.

The theory of reactive designs is of particular importance to the \Circus language family. \Circus is a language for
description of concurrent processes that interact via channels in a similar way to CSP~\cite{Hoare85}. Different to CSP
though, each process has encapsulated state variables that can be manipulated using assignments. The state is isolated
from other processes and the only form of data sharing remains the channels. Typical constructs of \Circus include

\begin{itemize}
  \item event prefix $a \then P$: perform event $a$ and then behave the $P$;
  \item assignment $x := v$: assign expresssion $v$ to local state variable $x$;
  \item external choice $P \extchoice Q$: pick $P$ or $Q$ depending on the offered events;
  \item the deadlocked process $\Stop$: it can make no progress and offer no events;
  \item guarded process $g \guard P$: behaves like $P$ is $b$ is true, otherwise deadlocks.
\end{itemize}

\noindent \Circus also has operators usual in a programming language like sequential composition, if-then-else, iteration, and
recursion. Moreover it has operators for parallel composition of processes, including explicit event sharing, and also
event abstraction. \Circus can properly be called a contract-based language, in as much as every construct of the
language can be described using a reactive design~\cite{Oliveira2005-PHD,Oliveira&09}.

Woodcock~\cite{Woodcock08} considers the top element of the lattice of reactive designs: miracle of reactive processes:
$\healthy{R}(\true \shows \false)$. This is the reactive design that is always guaranteed to terminate if it is started,
and when it does terminate, it achieves the impossible. He explores consequences of having such a process in combination
with some of the other operators in a process algebra. Its effect in the language is to prune away behaviour. For
example, the process
$$
  a \then \Miracle = \healthy{R}(\true \shows tr' = tr \land a \notin ref' \land wait' \land v'=v)
$$
If properly started, this process nevers refuses the event $a$, but the event never happens, since the resulting
behaviour would be miraculous. Perhaps more useful is the interaction with external choice:
$$
  a \then Skip \extchoice \Miracle =
  \healthy{R}(\true \shows \lnot wait' \land tr' = tr \cat \langle a \rangle \land v'=v)
$$
This process terminates immediately, having performed the event $a$. There is no state in which the process is waiting
for the environment to perform $a$, it simply happens instantly. Intuitively, we can think of this as an urgent
event. Woodcock suggests a couple of practical applications for miracles: ordered simultaneous events, where a second
event follows urgently on the heels of a first event
$$
  a \then (b \then Skip \extchoice \Miracle)
$$
and a hard deadline operator for timed CSP:
$$
  (a \then Skip) \timeout{10} \Miracle
$$
Here, the event $a$ is offered to the environment. If the environment fails to engage in this event before 10 seconds
have elapsed, then the process times out and behaves like a miracle. But this is impossible behaviour and there is no
alternative to meeting the deadline.

Butterfield et al.~\cite{BGW09} study the problem of state visibility in an imperative process algebra, noting that the
observation of program state is miraculous while waiting for an external choice to be resolved for $\healthy{R3}_c$
predicates. In this work he replaces the standard healthiness condition $\healthy{R3}$ with a variant called
$\healthy{R3}_h$, that causes internal state updates to be abstracted in intermediate obervations, that we shall utilise
in Section~\ref{sec:grd}.


==> sec/foundations.tex <==
Our theory of reactive contracts depends on a number of algebraic theorems for the UTP's predicate and relational
calculus, which we cover in this section. Many of this theorems are already well known, but we have mechanised them in
Isabelle/UTP or as part of the \textsf{HOL-Algebra} package~\cite{HOL-Algebra}, that we have contributed several
theorems to. Our main result about continuous healthiness conditions is, we believe, novel in its presentation.

The alphabetised predicate calculus is the foundational model into which all higher level models of computation are
embedded. It provides the usual operators of first-order logic, including conjunction ($\land$), disjunction ($\lor$),
negation ($\neg$), and quantification ($\exists$ / $\forall$). The calculus also has typed variables and expressions,
which includes equality, and operators from set theory and arithmetic, amongst other common mathematical theories. From
the stand-point of our Isabelle embedding, we permit any expression that can be expressed in HOL to be lifted into the
UTP predicate calculus. 

The majority of other operators, in particular those from relational calculus, can then be expressed in terms of the
core predicate calculus. The predicate calculus is supported by a number of important algebraic theories. In particular
we can prove that predicates form (1) a Boolean Algebra, (2) a Complete Distributive Lattice, (3) a Cylindrical
Algebra~\cite{Tarski71}, which governs the quantifiers, (4) a Complete Boolean Algebra, and (5) a Relation
Algebra~\cite{Tarski41}.

UTP theories exist as (non-empty) subsets of the domain of alphabetised predicates which have a set of syntactically
valid alphabets and are closed under an idempotent function that characterises its healthiness conditions. Usually a UTP
prescribes a number of observational variables that must be present, though leaves open the possibility for additional
variables. Indeed, this is central to theory extension and composition, whereby different theoretical aspects are
characterised by disjoint observational variables. In order to consider the domain of healthy predicates, and also
consider recursive and iterative behaviours, we need to reason about fixed-points of the healthiness functions which
requires that we consider lattice theory.

\begin{definition}[Complete lattices]
  A partially ordered set ($(\theory{P}, \sqsubseteq)$) is a complete lattice provided every of subset $A \subseteq
  \theory{P}$ has a greatest lower bound ($\bigsqcap A$) and least upper bound ($\bigsqcup A$). These must satisfy the
  following laws:
  \begin{align*}
     P \sqsubseteq (\bigsqcap S) &~~\textit{iff}~~ (P \sqsubseteq X ~~\textit{for all}~~ X ~~\textit{in}~~ S) \tag{L1} \\
     (\bigsqcup S) \sqsubseteq Q  &~~\textit{iff}~~ (X \sqsubseteq Q ~~\textit{for all}~~ X ~~\textit{in}~~ S) \tag{L2}
  \end{align*}
   
  \noindent We will often abbreviate binary versions of these operators: $P \sqcap Q \defs \bigsqcap \{P,Q\}$ and $P \sqcup Q
  \defs \bigsqcup \{P,Q\}$.
\end{definition}

\noindent We can then, in particular, show that the set of UTP predicates forms a complete lattice.

\begin{theorem}[UTP predicates complete lattice]
  UTP predicates form a complete lattice with $\bigsqcap S \defs \bigvee S$ and $\bigsqcup S \defs \bigwedge S$
\end{theorem}

\noindent If the healthiness function of a theory is monotonic then it the theory forms a complete lattice by the
following well known theorem, which we have mechanised as part of the \textsf{HOL-Algebra}~\cite{HOL-Algebra} library:

\begin{theorem}[Knaster-Tarski fixed points] \label{thm:knaster-tarski} Given a complete lattice $(\theory{L}, \le)$ and
  a monotone function $F : \theory{L} \to \theory{L}$, the set of fixed points of $F$, defined as $\theory{P} \defs \{ X \in \theory{L} |
  F(X) = X \}$, also forms a complete lattice $(\theory{P}, \le)$.
\end{theorem}

\noindent Since complete lattices have a least and a greatest element, a corollary of this theorem is that there exists
least and greatest fixed points of $F$, namely $\thlfp{L}~F \defs \thtop{P}$ and $\thgfp{L}~F \defs \thtop{P}$. In the
UTP, these are called the weakest and strongest fixed points with $(P \le Q) \defs (P \sqsubseteq Q)$. If $F$ is also
idempotent, then we also have it that $\theory{P} = \{ F(X) | X \in \theory{L} \}$, that is the image of $\theory{L}$
under $F$, and thus $\thtop{P} = f(\thtop{L})$ and $\thbot{P} = f(\thbot{L})$. The top and bottom elements correspond to
most and least determinisitc programs in the refinement lattice, which can be thought of as a miraculous program and an
erroneous program, respectively. Since alphabetised predicates form a complete lattice, we can derive the following
result.

\begin{theorem}[UTP theory lattice] \label{thm:utp-lattice} Given a UTP theory $\theory{T}$, whose healthiness function
  $\healthy{H}$ is idempotent and monotone, then $(\theory{T}, \sqsubseteq)$ forms a complete lattice with 
  \begin{align}
    \thsup{T} ~ A &~~\defs~~ \healthy{H}(\bigsqcup A) & \textit{provided}~~ A \subseteq P \\
    \thinf{T} ~ A &~~\defs~~ \healthy{H}(\bigsqcap A) & \textit{provided}~~ A \subseteq P \\
    \thtop{T}   &~~\defs~~ \healthy{H}(\false) \label{thm:utp-lattice-top} \\
    \thbot{T}   &~~\defs~~ \healthy{H}(\true)
  \end{align}
  Moreover, we obtain operators for calculating weakest and
  strongest fixed points in this lattice, $\thlfp{T}$ and $\thgfp{T}$, with the following laws for unfolding fixed points:
  \begin{itemize}
    \item $\thlfp{T}~F = F (\thlfp{T}~F)$ provided that $f : \theory{T} \to \theory{T}$ and $F$ is monotonic;
    \item $\thgfp{T}~F = F (\thgfp{T}~F)$ provided that $f : \theory{T} \to \theory{T}$ and $F$ is monotonic.
  \end{itemize}
We will sometimes write $\thlfp{T} X @ P(X)$ and $\thgfp{T} X @ P(X)$ to abbreviate $\thlfp{T} (\lambda
X @ P(X))$ and $\thgfp{T} (\lambda X @ P(X))$, respectively.
\end{theorem}

\noindent Thus, from the fact a healthiness condition is monotonic and
idempotent a large number of results can be obtained, for example:
\begin{theorem}[UTP theory lattice laws]
\begin{align}
  P &~~\refinedby~~ \thtop{T} & \text{provided}~~ \healthy{H}(P) = P \\
  \thbot{T} &~~\refinedby~~ P & \text{provided}~~ \healthy{H}(P) = P \\
  \thsup{T} A &~~\refinedby~~ \thsup{T} B & \text{provided}~~ A \subseteq B \\
  \thlfp{T} ~ X @ X &~~=~~ \thbot{T} \\
  \thlfp{T} ~ X @ P &~~=~~ P & \text{provided}~~ X ~~\text{does not appear in}~~ P
\end{align}
\end{theorem}
\noindent In our example theory we have $\thtop{T} = HT(\false) = \false$, and $\thbot{T} = HT(\true) = time \le time'$,
that is an erroneous program can have any behaviour, but time can only advance. Beyond monotonic UTP theories, we can
also consider the class of continuous healthiness conditions, which are infimum preserving:
\begin{definition}[Continuous healthiness conditions]
  A healthiness condition \healthy{H} is said to be continuous if it satisfies $\healthy{H}(\bigsqcap A) = \bigsqcap \{
  \healthy{H}(P) | P \in A \}$ for $A \neq \emptyset$.
\end{definition}
\noindent Every continuous healthiness condition is also monotonic and thus likewise induces a complete
lattice. However, continuity also means that the theory infimum ($\thinf{T}$) is in fact the same operator as the
alphabetised predicate infimum ($\bigsqcap$), meaning programs can be constructed using these operators. This means that
a number of additional laws can be transplanted into the theory, some of which are illustrated below.
\begin{theorem}[Continuous theory laws] \label{thm:contthm}
\begin{align}
  P \intchoice P         &~~=~~ P \\
  P \intchoice Q         &~~=~~ Q \intchoice P \\
  P \intchoice (Q \intchoice R) &~~=~~ (P \intchoice Q) \intchoice R \\
  \thbot{T} \intchoice P &~~=~~ \thbot{T} & \text{provided}~ \healthy{H}(P) = P \\
  \thtop{T} \intchoice P &~~=~~ P & \text{provided}~ \healthy{H}(P) = P \\
  \thlfp{T} X @ F(X) & ~~=~~ \mu X @ F(\healthy{H}(X)) \label{thm:contthm-lfp}
\end{align}
\end{theorem}
Of particular interest here is Theorem~\ref{thm:contthm-lfp} that shows how a theories weakest fixed-point operator can
be rewritten to the alphabetised predicate weakest fixed-point. The requirement is that continuous healthines condition
$\healthy{H}$ be applied after each unfolding of the fixed-point to ensure that the function $F$ is only ever presented
with a healthy predicate.

Healthiness conditions in the UTP are often built from several component functions, e.g. $\healthy{H} \defs
\healthy{H}_1 \circ \healthy{H}_2 \circ \healthy{H}_3$. That being the case, monotonicity and idempotence
of the overall healthiness condition can be obtained by composition as the following theorem shows.

\begin{theorem}[UTP heathiness conditions] \label{thm:hcond-comp} Given a UTP theory whose healthiness condition is built from $n$
  constituents, $\healthy{H} \defs \healthy{H}_1 \circ \cdots \circ \healthy{H}_n$, then:
  \begin{itemize}
    \item $\healthy{H}$ is idempotent provided $\healthy{H}_1 \cdots \healthy{H}_n$ are all idempotent, and each pair
      commutes, i.e. $\forall i,j < n @ H_i \circ H_j = H_j \circ H_i$;
    \item $\healthy{H}$ is monotone provided $\healthy{H}_1 \cdots \healthy{H}_n$ are all monotone;
    \item $\healthy{H}$ is continuous provided $\healthy{H}_1 \cdots \healthy{H}_n$ are all continuous.
  \end{itemize}
\end{theorem}


==> sec/lifting.tex <==
Aside from unifying reactive languages, our contracts also allow us to link them with imperative specification languages
like VDM and Z. In such notations, systems are specified in terms of operations that are formulated as relations on
state variables. As mentioned in Section~\ref{sec:related}, the theory of designs can be applied to unifying such
specification formalisms. Thus, in this section we formulate a link between the theory of designs and reactive designs,
which enables embedding imperative programs and specification languages into reactive contracts. Namely, we specify functions for
converting designs to reactive designs, and vice-versa.

\begin{definition}[Lifting Functions]
  \begin{align*}
    \healthy{R}_D(P) ~~\defs~~~& \Rs(\preD{P} \shows false \wcond (\trace = \langle\rangle \land \postD{P}) \\
    \healthy{D}_R(Q) ~~\defs~~~& (\preR{Q})[tr'/tr] \shows (\postR{Q})[tr'/tr]
  \end{align*}
\end{definition}

\noindent Here, $P$ is a normal UTP design on state variables alone: its alphabet consists of $ok$, $ok'$, $st$, and
$st'$, and it is $\healthy{N}$ healthy. $Q$ is any reactive design predicate. The function $\healthy{R}_D$ embeds a
state-variable design into a reactive design by copying the precondition, setting the pericondition to $\false$, since
there are no intermediate observations, and conjoining the postcondition with $\trace = \langle\rangle$ so that no
events occur. If $P$ is a normal design, then it follows that $\healthy{R}_D(P)$ is a normal stateful reactive design,
since the precondition will consider only unprimed state variables and not the trace.

We also introduce the function $\healthy{D}_R$ as its inverse: it constructs a normal design that ignores the
pericondition and permits no trace behaviour by substituting $tr$ for $tr'$. We can show that, for any normal design
$p \shows Q$, $\healthy{D}_R$ is the inverse of $\healthy{R}_D$.

\begin{theorem}[Lifting Theorems]
  \begin{align}
    \healthy{D}_R(\healthy{R}_D(p \shows Q)) ~=~~~& p \shows Q \\
    P \refinedby Q ~ \implies ~ \healthy{R}_D(P) ~\refinedby~~~& \healthy{R}_D(Q)
  \end{align}
\end{theorem}

\noindent A corollary of this theorem is that $\healthy{R}_D$ is an injective function: every normal design has a
corresponding unique reactive design. $\healthy{R}_D$ is also monotonic, meaning refinement of a lifted imperative
design can be determined by refinement of the design itself. Finally, we demonstrate some homomorphism laws of
$\healthy{R}_D$.

\begin{theorem}[Lifting Homomorphisms]
  \begin{align*}
    \healthy{R}_D(\topD) &= \Miracle \\
    \healthy{R}_D(\botD) &= \Chaos \\
    \healthy{R}_D(\IID)  &= \IIsrd \\
    \healthy{R}_D(P \intchoice Q) &= \healthy{R}_D(P) \intchoice \healthy{R}_D(Q) \\
    \healthy{R}_D(P \infixIf b \infixElse Q) &= \healthy{R}_D(P) \infixIf b \infixElse \healthy{R}_D(Q) \\
    \healthy{R}_D(P \relsemi Q) &= \healthy{R}_D(P) \relsemi \healthy{R}_D(Q) \\
    \healthy{R}_D(\assignsD{\sigma}) &= \assignsR{\sigma}
  \end{align*}
\end{theorem}

\noindent Lifting the design top and bottom yields the reactive design top and bottom, as expected, and lifting the
design identity yields the reactive identity. Moreover, $\healthy{R}_D$, as expected, distributes through internal
choice, conditional, and sequential composition. Finally, lifting the design assignment yields the reactive assignment.


==> sec/mech.1.tex <==

In this section we give a brief overview of the mechanisation work in Isabelle/UTP~\cite{Foster16a,Zeyda16}, which has supported
the development of our theory of reactive contracts, and has allowed us to turn these theories into a prototype
verification tool. Our theory hierarchy was developed almost entirely mechanically; whilst we used whiteboard proofs for
the main high-level theorems, all the low-level lemmas were proved automatically using the proof tactics we developed
for the relational calculus. This significantly helped our theory engineering to progress at a speedy pace, thus aiding
the exploration of theory properties and discovery of missing assumptions in our theorems. It thus improved the
precision of our theories by preventing formalisation gaps in proofs, and of course improves overall confidence in the
correctness of our theorems. Moreover, the mechanised theorems for contract calculation given in
Section~\cite{sec:contracts} have also been compiled into a proof tactic for contract verification.

\subsection{Repository Overview}

\subsection{Isabelle/UTP}

All definitions and theorems have been mechanised in our UTP theorem prover, Isabelle/UTP~\cite{Foster16a,Zeyda16},
which is a semantic embedding of the UTP predicate and relational calculus in Isabelle/HOL~\cite{Isabelle}. We will here
give a brief overview of the mechanisation, and highlight some key technical details which have be thus far
elided.

Broadly speaking the syntax mirrors that of the mathematical account presented in this paper, with a few notable
exceptions. In particular, the handling of alphabets utilises the Isabelle type system to ensure well-formedness of
expressions, but requires insertion of explicit alphabet coercions. Moreover, for our UTP expression model we sometimes
want to reuse operator names already defined in HOL such as $+$, $\le$, and $=$. Sometimes this can be achieved through
polymorphic overloading, as is the case for $+$ and also numerical representations, which are both handled through the
type class mechanism. This does not work for $\le$ as the type does not fit the polymorphic pattern, and so we have to
add a subscript: $x \le_u y$. This is also true of several other operators, including $=$ which becomes $=_u$ so as not
to clash with HOL's operator which we often use for expressing algebraic laws.

Alphabetised predicates are modelled by a parametric type
$\alpha\ \upred \defs (\alpha \Rightarrow \mathbb{B})$, where $\alpha$ is the alphabet type. A predicate is thus a
function that states whether a particular state binding of the alphabet satisfies it. For example,
$\true \defs \lambda x @ \mathit{True}$, where $\mathit{True}$ is HOL's true, since any binding satisfies it. All the
propositional logic operators of the UTP's predicate calculus are obtained by similar lifting of HOL equivalents, for
example $P \land Q \defs \lambda x @ P(x) \land_{\tiny H} Q(x)$, where the right-hand side has the HOL operator. Our
predicate model is thus inherently \textbf{alphabet polymorphic}: predicates are open to extension and proven laws can
be instantiated to a variety of alphabets. This is important for our unifying theory of contracts where additional
variables such as $ref'$ may or may not be present, but generic laws still apply. Alphabetised relations are simply
predicates whose alphabet is a product space:
$$(\alpha, \beta)\ \urel \defs (\alpha \times \beta)\ \upred$$

Variables are modelled using lenses~\cite{Foster09,Foster16a}; these are projections that identify a particular region
of the alphabet. A lens $x : \tau \lto \alpha$ shows how to project the variable data of type $\tau$ out of the alphabet
$\alpha$. The behaviour of a lens is constrained by a number of algebraic laws~\cite{Foster16a}. Lenses can be tested
for observational equivalence using $x \lequiv y$, for $x : \tau_1 \lto \alpha$ and $y : \tau_2 \lto \alpha$ (i.e. with
potentially different view types, but the same source), containment using the sublens relation $x \lsubseteq y$, and
observational difference using $x \lindep y$, which we call lens independence. 

Relational variables, with a product alphabet, can be constructed using lens compositions. The initial value of $x$ is
obtained by $\lfst \lcomp x$, and the final value by $\lsnd \lcomp x$. Lenses $\lfst$ and $\lsnd$ select the first and
second part of a product, respectively, and the composition operator $\lcomp$ is analogous to function composition. In
Isabelle/UTP initial and final variables are written as \verb|$x| and \verb|$x`|, respectively. Also useful for dealing
with relational lenses is the product lens $a \lprod b$ that point-wise composes $a : \alpha \lto \gamma$ and
$b : \beta \lto \delta$, to produce a lens of type $\alpha \times \beta \lto \gamma \times \delta$.

One can also check whether a given predicate $P$ depends on a particular lens $x$ using the unrestriction predicate
$\unrest{x}{P}$, which means that $P$'s truth-valuation is unchanged if $x$ is changed. Unrestriction thus effectively
gives us a semantic characterisation of whether a variable is present in a predicate or not. It distributes through
the predicate operators as expected, for example $$\unrest{x}{P} \land \unrest{x}{Q} \implies \unrest{x}{(P \land Q)}$$

Since types are used to model alphabets, modification by adding or removing variables means that we must perform a type
coercion. We implement two operators in Isabelle/UTP: alphabet extrusion ($P \aext a$) and alphabet restriction
($Q \ares a$), for $a : \beta \lto \alpha$, $P : \beta\ \upred$, and $Q : \alpha\ \upred$. Lens $a$ shows how one
alphabet $\beta$ can be embedded into another alphabet $\alpha$. Thus alphabet extrusion modifies $P$, whose alphabet is
$\beta$ to have the ``larger'' alphabet $\alpha$, and restriction is the converse of this. Alphabet extrusion is a
lossless operation, whereas restriction can potentially lose information about removed portions of the
alphabet. Following an extrusion, $P \aext a$, it is guaranteed that an lens independent of $a$ is unrestricted. This is
because $P$ exclusively talks about alphabet $\beta$, and not other parts of the larger $\beta$:
$$x \lindep a \implies \unrest{x}{(P \aext a)}$$

For reactive designs, we use alphabet extrusions to impose constraints such as ``$ok$ and $wait$ are not
mentioned''. This is done through our own \textbf{alphabet} command in Isabelle -- an extension of the record package
that also creates a lens for each field. Moreover, like the record package, we utilise parametric polymorphism and the
associated subtyping mechanism such that alphabets can be extended by the addition of field lenses. The alphabet of
designs is described by the type $\alpha\,\textit{des}$, which consists of the single lens
$ok : \mathbb{B} \lto \alpha\ \textit{des}$. Parameter $\alpha$ can be used to extend the alphabet with further
variables. 

In this way, we create the extended alphabet type $(\sigma, \mathcal{T}, \alpha) \textit{rsp}$ for stateful reactive
processes, where $\sigma$ is the variable state-space, $\mathcal{T}$ is a trace algebra type, and $\alpha$ permits
further extension. In addition to $ok$ it also has lenses
\begin{itemize}
  \item $wait : \mathbb{B} \lto (\sigma, \mathcal{T}, \alpha)\ \textit{rsp}$;
  \item $tr : \mathcal{T} \lto (\sigma, \mathcal{T}, \alpha)\ \textit{rsp}$; and
  \item $st : \sigma \lto (\sigma, \mathcal{T}, \alpha)\ \textit{rsp}$.
\end{itemize}

State variables will all be sublenses of $st$, meaning they exclusively observe that portion of the state-space. Thus,
if we have a homogeneous relation $R$ on state variables only of type $(\sigma, \sigma)\ \urel$, then we can lift this
into a relation on the alphabet $(\sigma, \mathcal{T}, \alpha) \textit{rsp}$ via alphabet extrusion
$P \aext (st \lprod st)$, which we give the notation $\lceil R \rceil_S$. This predicate has $ok$, $wait$, $tr$ etc. all
unrestricted, and thus we are using the type system to encode alphabet provisos. Similarly, we provide such lifting
operators for preconditions on the state-space, $\lceil P \rceil_{S<}$, where $P : \sigma\ \upred$.

\begin{figure}
  \includegraphics[width=11.8cm]{figures/Pay_contract}

  \caption{Calculating the contract of $Pay$ in Isabelle/UTP}
  \label{fig:PayContract}
\end{figure}

Thus, in many of the mechanised versions of the reactive design laws such coercions must be manually inserted. For
example, in Theorem~\ref{thm:mondexcontract}, where we calculate the contract of the $Pay$ action, the last disjunct of
postcondition $P_3$, the assignment where the accounts are debited and credited, actually has
$$\lceil accts := accts(i \mapsto accts(i) - n, j \mapsto accts(j) + n) \rceil_S$$ in the mechanisation. This is 
illustrated in the screenshot in Figure \ref{fig:PayContract}. Here, $accts$ is actually a lens of type
$\textit{int}\,\textit{list} \lto \textit{st-mdx}$ in Isabelle, where \textit{st-mdx} is the state-space type, and thus
must be lifted.

\subsection{Parallel-by-Merge}

Mechanisation of parallel-by-merge posed some specific technical challenges, and thus we will summarise how it
works. Since alphabets are types in Isabelle/UTP, the type of each variable is sensitive to alphabet extension which
introduces some notational issues. When constructing a parallel composition ($P \parallel_M Q$) it is necessary to
extend the alphabet to include three copies of the variables: indexed varieties for $P$ and $Q$, and the initial value
of variables. If $P$ and $Q$ are both homogeneous relations of type $(\alpha, \alpha)\,\urel$ then the merge predicate
$M$ essentially has type $(\alpha \times \alpha \times \alpha, \alpha)\,\urel$, since it merges three copies of the
state. For reasons of convention, the initial state is the first $\alpha$, and the indexed states are the second and
third, respectively.

Unfortunately, that means that unlike in mathematical UTP we cannot refer to the initial values of variables using the
standard undecorated variable notation (\verb|$x|), as such as construction has type $\alpha \lto (\alpha \times
\alpha)$, when we actually want to project from a source type $\alpha \times \alpha \times
\alpha$. Thus we have to introduce three notations, \verb|$x|$_<$, \verb|$0-x|, and \verb|$1-x|, for the three
components. We also implement the renaming notations $\psep{P}{0}$ and $\psep{Q}{1}$ that both perform alphabet
extrusion, converting both to have type $(\alpha, \alpha \times \alpha \times \alpha) \urel$ to match the output with
the input of the merge predicate. The final representation of $P \parallel_M Q$ is
$(\psep{P}{0} \land \psep{Q}{1} \land v' = v_<) \relsemi M$ which has type $(\alpha, \alpha)\,\urel$ as expected.

This technicality also has an impact on the formalisation of the healthiness conditions for merge predicates. In
mathematical UTP, we can simply reuse $\healthy{R1}$, $\healthy{R3}_h$, and other healthiness conditions. Here, we have
to create variants that refer to the explicit initial variables instead, which we give names like $\healthy{R1m}$ whose
definition is $tr_{<} \le tr'$. Using these, we then prove all the laws for parallel composition and reactive
designs. These healthiness conditions, it should be stressed, are semantically equivalent modulo variable renamings. Of
course, this isn't the case for $\healthy{R2}_c$ which as we have previously showed~\cite{Foster17a} requires
modification anyway.

\subsection{Reactive Design Tactics}

One particular aim of this work has been to support a high level of automated reasoning for reactive contracts. This has
involved the creation of new tactics and utilisation of a number of existing tactics. The initial particular problem to
be solved is bridging the gap between UTP predicates and HOL predicates which are distinct types, albeit strongly
related. In particular, the majority of operators of the former are defined, via the \textbf{lifting}
package~\cite{Huffman13}, in terms of operators of the latter. The major difference is the addition of lenses which
accounts for the alphabet or state-space not implicitly present in HOL predicates.

Our approach to reasoning about alphabetised predicates and relations therefore extends the approach we first described
in~\cite{Foster14}. The basic approach is two step: firstly apply the transfer tactic to interpret a UTP predicate to a
HOL predicate, and secondly apply Isabelle/HOL's built in automated reasoning tactics, such as \textit{auto},
\textit{sledgehammer}, and \textit{nitpick}. We've now also extended this approach to provide explicit support for
lenses. Each record lens can be collapsed and rewritten to a HOL variable with a similar name. Effectively this means
that reasoning about UTP predicates and relations can often be reduced to reasoning about HOL predicates, which of
course improves automation. In particular, for relations, proof reduces to a satisfiability problem since sequential
composition boils down to existential quantification. We provide tactic \textbf{pred-auto} which uses this approach,
combined with HOL's \textbf{auto} to deal with predicate conjectures, and \textbf{rel-auto} to deal with relational
conjectures.

Reasoning about predicates and relations in this is indeed powerful, but it becomes unwieldy when dealing with very
complex definitions, particularly our reactive contracts. Each reactive contract is written in terms of the $\Rs$
healthiness condition, and the design turnstile, which adds a large overhead particularly when dealing with large
composite definitions. Thus we develop an additional tactic, based on the algebraic laws of Sections~\ref{sec:contracts}
and \ref{sec:grd}. The tactic can be used to prove (or refute) refinement conjectures of the form $P \sqsubseteq Q$ for
two reactive design contracts. Moreover, through application of antisymmetry, we can also use it to prove equality
conjectures.

The process has three stages:

\begin{enumerate}
\item \textbf{Calculate and simplify reactive design contracts}. The algebraic laws of reactive designs are applied to
  convert a composite reactive contract into a monolithic one of the syntactic form $\rc{P}{Q}{R}$. This of course
  necessitates that appropriate calculation theorems have been proved and are already available;
\item \textbf{Apply the refinement theorem}. Theorem~\ref{thm:rdesrefine} is applied to break the refinement conjecture
  into three proof obligations about the pre-,peri-, and postconditions.
\item \textbf{Apply relational transfer and reasoning tactic}. The three proof obligations are purely relational, do not
  refer to observational variables $ok$ and $wait$, and thus are much more lightweight in nature. Thus we can now apply
  \textbf{rel-auto}, and potentially other HOL tactics, to try and complete the proof. Of course, we can also at this
  point try to generate a counterexample, which can be traced back to a fault in the pre-,peri-, or postcondition.
\end{enumerate}

We have found this approach extremely useful for automated reasoning, and it has been used to valid all the example
calculations, in particular those related to the MiniMondex example\footnote{See
  \url{https://github.com/isabelle-utp/utp-main/blob/master/tutorial/utp_csp_mini_mondex.thy} for our complete
  mechanised theory}.



